Lattice-type self-similar sets with pluriphase generators fail to be Minkowski measurable

A long-standing conjecture of Lapidus claims that under certain conditions, self-similar fractal sets fail to be Minkowski measurable if and only if they are of lattice type. The theorem was established for fractal subsets of $\mathbb{R}$ by Falconer, Lapidus and v.~Frankenhuijsen, and the forward direction was shown for fractal subsets of $\mathbb{R}^d$, $d \geq 2$, by Gatzouras. Since then, much effort has been made to prove the converse. In this paper, we prove a partial converse by means of renewal theory. Our proof allows us to recover several previous results in this regard, but is much shorter and extends to a more general setting; several technical conditions appearing in previous versions of this result have now been removed.

==> monophase.tex <==
\noindent$\negsp[5]$\fbox{\scalebox{0.83}{\begin{minipage}{6in}
Do we keep the following section or not? 

It seems like Cor.~\ref{cor:severalmonophase} is just immediate from Theorem~\ref{thm:main-result} now, and the proof is almost the same as well. On the other hand, it seems a waste to throw it away.
\end{minipage}}}

\subsection{The monophase case} ~\\

\begin{cor}\label{cor:severalmonophase}
	In addition to the prerequisites in Theoerem \ref{thm:subresult} assume that $\gl_d(\Gamma\setminus\inn\Gamma)=0$ and that $\inn \gG$ has finitely many connected components, each of which is monophase. %$\gl_d(\Gamma\setminus\inn\Gamma)=0$ and that the interior $\inn\Gamma$ of $\Gamma$ has finitely many connected components, denoted by $G^1,\ldots, G^Q$ with $Q\in\mathbb N$, so that $\inn\Gamma=\bigcup_{q=1}^Q G^q$ and $G^q\neq\emptyset$ for $q=1,\ldots,Q$. 
	%Set $g^q\defeq \sup\{d(x,F)\mid x\in G^q\}$ and suppose that $\ge\mapsto\gl_d(F_{\ge}\cap G^q)$ is polynomial on $(0,g^q]$. 
	Then $F$ is not Minkowski measurable.
\end{cor}

\begin{proof}
	Let $\{\gG^q\}_{q=1}^Q$ denote the connected components of $\gG$, and let $g^q\defeq \sup\{d(x,F)\mid x\in \gG^q\}$. The new hypothesis then states that for each $q = 1,\ldots,Q$, there exist real coefficients $\eta_0^q, \dots, \eta_{d-1}^q$ such that 
	\linenopax
	\begin{equation*}
	\gl_d(F_{\ge}\cap \gG^q)=\sum_{k=0}^{d-1}\eta_k^q \ge^{d-k}\quad\text{for}\ \ge\in(0,g^q].
	\end{equation*}
	Note that the summation ends at $d-1$ since $\lim_{\ge\to 0}\gl_d(F_{\ge}\cap \gG^q)=0$. For $\ge>g^q$ we have $\gl_d(F_{\ge}\cap \gG^q)=\gl_d(\gG^q)$. 
	
	We make use of the result of Theorem \ref{thm:subresult}. For showing that $F$ is not Minkowski measurable, it thus suffices to show that the periodic function $p(\ge)$ of \eqref{eqn:p(e)} is non-constant. 
	%From the disjoint union $\Gamma=\bigcup_{q=1}^Q \gG^q\cup(\Gamma\setminus\inn\Gamma)$ and the assumption $\gl_d(\Gamma\setminus\inn\Gamma)=0$ 
	From \eqref{eqn:open-tiling}, we deduce that
	\linenopax
	\begin{align*}
	p(\ge) &= \ge^{D-d}\sum_{q=1}^Q \sum_{\ell\in\mathbb Z} r^{\ell(D-d)} \gl_d(F_{r^{\ell}\ge}\cap \gG^q).
	%p_2(\ge)&\defeq\ge^{D-d}\sum_{\ell\in\mathbb Z}r^{\ell(D-d)}\gl_d(F_{r^{\ell}\ge}\cap (\Gamma\setminus\inn\Gamma)).
	\end{align*}
Therefore,
	\linenopax
	\begin{align*}
	p(\ge)
	&=\ge^{D-d}\sum_{q=1}^Q\sum_{\ell\in\mathbb Z}r^{\ell(D-d)}\left[\sum_{k=0}^{d-1}\eta_k^q(r^{\ell}\ge)^{d-k}\one_{(0,g^q]}(r^{\ell}\ge)+\gl_d(\gG^q)\one_{(g^q,\infty)}(r^{\ell}\ge)\right].
	\end{align*}
	Set $\tilde{L}^q(\ge)\defeq \left\lceil\log_r\tfrac{g^q}{\ge}\right\rceil$, where $\lceil x\rceil$ denotes the smallest integer greater than or equal to $x$, so that $\lceil x\rceil$ rounds up. Upon noting that $r^{\ell}\ge\leq g^q$ iff $\ell\geq\tilde{L}^q(\ge)$ for $\ell\in\mathbb Z$ we conclude
	\linenopax
	\begin{align*}
	p(\ge)
	&=\ge^{D-d}\sum_{q=1}^Q\left[\sum_{k=0}^{d-1}\eta_k^q\ge^{d-k}\sum_{\ell=\tilde{L}^q(\ge)}^{\infty}r^{\ell(D-k)}
	+\gl_d(\gG^q)\sum_{\ell=-\infty}^{\tilde{L}^q(\ge)-1}r^{\ell(D-d)}\right]\\
	&=\ge^{D-d}\sum_{q=1}^Q\left[\sum_{k=0}^{d-1}\eta_k^q\ge^{d-k}\frac{r^{\tilde{L}^q(\ge)(D-k)}}{1-r^{D-k}}
	+\gl_d(\gG^q)\frac{r^{d-D}(1-\tilde{L}^q(\ge))}{1-r^{d-D}}\right].
	\end{align*}
	Following usual convention we set $\eta_d^q\defeq-\gl_d(\gG^q)$, which yields
	\linenopax
	\begin{equation}\label{eq:p-monophase}
	p(\ge)
	= \ge^{D}\sum_{k=0}^{d}\ge^{-k}\underbrace{\sum_{q=1}^Q\eta_k^q\frac{r^{\tilde{L}^q(\ge)(D-k)}}{1-r^{D-k}}}_{\eqdef \tilde{\eta}_k(\ge)}.
	\end{equation}
	Since $p$ is multiplicatively periodic with multiplicative period $r$ it suffices to show that $p$ is non-constant on an interval of multiplicative length $r$, say $(r,1]$ for showing that $p$ is non-constant. On $(r,1]$, the function $\tilde{L}^q$ is piecewise constant with at most one point of discontinuity. Therefore, on $(r,1]$, the function $\tilde{\eta}_k$ is piecewise constant with at most $Q$ points of discontinuity. Moreover, these points of discontinuity coincide for all $k=0,\ldots,d$. Thus, we can partition $(r,1]$ into a finite number of intervals, on each of which every $\eta_k$ is constant. Restricted to any of these intervals $\ge\mapsto\ge^{-D}p(\ge)$ thus is a polynomial in $\ge^{-1}$ with at least one non-zero coefficient, namely the one corresponding to the index $d$, since $\eta_d^q=-\gl_d(\gG^q)<0$ for every $q=1,\ldots,Q$. Since the monomials are linearly independent, it now follows that $p$ cannot be constant.
\end{proof}

\begin{remark}\label{rmk:previous}
 Corollary \ref{cor:severalmonophase} is both a corollary to Theorem \ref{thm:subresult} and a special case of Theorem \ref{thm:main-result}. However, the assumptions which are additional to the ones in Theorem \ref{thm:main-result} simplify the proof significantly. Therefore, we state this simpler proof although the statement of Corollary \ref{cor:severalmonophase} is included in the one in Theorem \ref{thm:main-result}.\\
		 Under the additional assumption that $\bd O\ci F$, the setting in  Corollary \ref{cor:severalmonophase} can be viewed as having a finite number of connected monophase generators, namely $G^1,\ldots,G^Q$ in the sense of Remark \ref{rmk:pluriphase:generator}. The case of finitely many connected monophase generators has been dealt with in \cite[Theorem 2.38]{Kombrink:thesis}, and the proof of Corollary \ref{cor:severalmonophase} closely follows the proof of this result.
\end{remark}

\begin{remark}
	The proof of Corollary \ref{cor:severalmonophase} is even simpler if we assume that $\Gamma$ is monophase (i.\,e. $Q=1$) rather than a union of monophase sets. Then it is already clear from \eqref{eq:p-monophase} that $p$ is non-constant:
	By definition $\tilde{L}\defeq \tilde{L}^1$ is constant on any interval of the form $(r^{s+1}g,r^s g]$ with $s\in\mathbb N$, where $g\defeq g^1$. Since $p$ is periodic, it suffices to work with $s=0$, in which case $\tilde{L}(\ge)=0$ for $\ge\in(rg,g]$. Thus, \eqref{eq:p-monophase} implies that $\ge\mapsto\ge^{-D}p(\ge)$ is a polynomial in $\ge^{-1}$ on $(rg,g]$ with at least one non-zero coefficient, namely $\tilde{\eta}_d(\ge)\equiv\eta_d^1/(1-r^{D-d})=-\gl_d(G^1)/(1-r^{D-d})>0$. Hence, $p$ cannot be constant on $(rg,g]$.
		
	Under the additional assumption that $\bd O\ci F$, the case $Q=1$ has been investigated in \cite{Minko}.
	This setting is known as the setting of a single connected monophase generator. The results in \cite{Minko} have been obtained by means of the theory of complex dimensions \cite{FGCD}. In comparison to the approach in \cite{Minko}, the proof that we present here, in Theorem \ref{thm:subresult} and Corollary \ref{cor:severalmonophase} (in conjunction with the preceding paragraph) is much shorter and simpler.
\end{remark}

\begin{remark}
	Under the additional assumptions that $O=\inn \langle F\rangle$, where $\langle F\rangle$ denotes the convex hull of $F$ and $\inn \langle F\rangle$ its interior, and that $Q=1$, the  statement of Corollary \ref{cor:severalmonophase} was obtained in \cite{Kocak1} by applying transformation theory to (tubular) zeta-functions. This approach is similar to the one in \cite{Minko} but the results were obtained independently.		
\end{remark}


\begin{proof}[Proof of Theorem \ref{thm:main-result}]
We prove that \eqref{eq:asympsum} is not constant. We know that $p(\ge)$ is periodic on $(0,g]$ but only given by formula \eqref{eq:asympsum} for $\ge \in (rg,g]$, so we have
\linenopax
\begin{align*}%\label{eqn:}
	p(\ge) 
	&= \ge^{D-d} \left[\frac{\gl_d(\Gamma)}{r^{D-d}-1} 
		+ \sum_{\ell = 0}^{\infty} r^{\ell(D-d)}  \sum_{k=0}^{d-1} \gk_k (r^\ell \ge)^{d-k} \right] \\
	%&= \ge^{D-d} \left[\frac{\gl_d(\Gamma) r^{-N(D-d)}}{r^{D-d}-1} 
%		+  \sum_{k=0}^{d-1} \gk_k \ge^{d-k} \sum_{\ell = -N}^{\infty} r^{\ell(D-k)}  \right] \\
	&= \ge^{D-d} \left[\frac{\gl_d(\Gamma) }{r^{D-d}-1} 
		+  \sum_{k=0}^{d-1} \gk_k \ge^{d-k} \frac{1}{1-r^{D-k}}  \right] \\
	&= \sum_{k=0}^{d} \frac{\ga_k}{1-r^{D-k}} \ge^{D-k},
\end{align*}
for $\ge \in (rg,g]$, where
\linenopax
\begin{align*}%\label{eqn:}
	\ga_k \coloneqq
	\begin{cases}
		\gk_k &k=0,1,\dots,d-1, \\
		-\gl_d(\Gamma) &k=d. \\
	\end{cases}
\end{align*}
Setting the derivative of $p(\ge)$ to 0 gives
\linenopax
\begin{align*}%\label{eqn:}
	p'(\ge) = \sum_{k=0}^{d} \frac{\ga_k \cdot (D-k)}{1-r^{D-k}} \ge^{D-k-1} = 0.
\end{align*}
Since the functions $\{\ge^{D-1},\ge^{D},\dots,\ge^{D-d-1}\}$ are linearly independent, %(note that $d-1 < D < d$), 
this implies $\ga_k = 0$ for $k=0,1,\dots,d$, which implies that $\gl_d(F_\ge \cap \Gamma)$ is identically 0 for \ge in the open interval $(rg, g]$, an obvious contradiction.
\end{proof}







